FineWeb-CLaR: Culture, Language, and Region Annotations for Benchmark-Aligned Corpus Auditing

Cultural evaluation coverage and robustness in language models are difficult to diagnose because pretraining corpora and cultural benchmarks are rarely indexed with comparable metadata. Benchmarks increasingly target culturally situated phenomena at the level of languages, regions, and locale-specific practices, while web-scale corpora are usually organized only by language. A shared culture-language-region layer makes these resources comparable, enabling audits of whether a target cultural phenomenon is represented in pretraining data, evaluated by benchmarks or both. To this end, we introduce FineWeb-CLaR, a large-scale annotated dataset derived from FineWeb and FineWeb-2 that places web documents on a shared culture-language-region axis for corpus auditing and benchmark alignment. FineWeb-CLaR annotates the full 30.9B-document collection from FineWeb and FineWeb-2 with URL-derived region labels and cultural-topic provenance. Our region resolver assigns a non-empty region to 25.61% of documents (7.92B). For cultural-topic analysis, we induce locale-specific topics and project them onto the 14 leaves of the Cultural Taxonomy of Liu et al. (2025), producing Locale Topic Distributions (LTDs) for corpus-side comparison. We also annotate 277 cultural NLP benchmarks with the same taxonomy, language coverage, and region coverage. Together, these resources enable direct comparison between corpus-side pretraining evidence and benchmark-side evaluation coverage.

==> figures/tab_country_languages.tex <==
% Auto-generated by latex/figures/gen_tikz.py -- do not edit by hand.
\begin{table*}[t]
\centering\tiny
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{@{}p{0.45cm}p{2.32cm}@{\hspace{6pt}}@{}p{0.45cm}p{2.32cm}@{\hspace{6pt}}@{}p{0.45cm}p{2.32cm}@{\hspace{6pt}}@{}p{0.45cm}p{2.32cm}@{\hspace{6pt}}@{}p{0.45cm}p{2.32cm}@{}}
\toprule
\textbf{CC} & \textbf{Main languages} & \textbf{CC} & \textbf{Main languages} & \textbf{CC} & \textbf{Main languages} & \textbf{CC} & \textbf{Main languages} & \textbf{CC} & \textbf{Main languages} \\
\midrule
\texttt{AD} & \texttt{cat} \texttt{spa} & \texttt{CW} & \texttt{nld} \texttt{pap} & \texttt{IN} & \texttt{asm} \texttt{ben} \texttt{eng} \texttt{guj} \texttt{hin} \texttt{kan} \texttt{kas} \texttt{kha} \texttt{kok}$^{\dagger}$ \texttt{mai} \texttt{mal} \texttt{mar} \texttt{nep}$^{\dagger}$ \texttt{ori}$^{\dagger}$ \texttt{pan} \texttt{san} \texttt{sat} \texttt{snd} \texttt{tam} \texttt{tel} \texttt{urd} & \texttt{MV} & \texttt{div} \texttt{eng} & \texttt{SM} & \texttt{ita} \\
\texttt{AE} & \texttt{ara}$^{\dagger}$ \texttt{eng} & \texttt{CY} & \texttt{ell} \texttt{eng} \texttt{tur} & \texttt{IQ} & \texttt{ara}$^{\dagger}$ \texttt{aze}$^{\dagger}$ \texttt{ckb} \texttt{eng} & \texttt{MW} & \texttt{eng} \texttt{nya} & \texttt{SN} & \texttt{bjt} \texttt{bsc} \texttt{dyo} \texttt{fra} \texttt{ful}$^{\dagger}$ \texttt{knf} \texttt{mey} \texttt{mfv} \texttt{sav} \texttt{snf} \texttt{srr} \texttt{tnr} \texttt{wol} \\
\texttt{AF} & \texttt{fas}$^{\dagger}$ \texttt{pus}$^{\dagger}$ \texttt{tuk} \texttt{uzb}$^{\dagger}$ & \texttt{CZ} & \texttt{ces} \texttt{deu} \texttt{eng} \texttt{slk} & \texttt{IR} & \texttt{aze}$^{\dagger}$ \texttt{fas}$^{\dagger}$ & \texttt{MX} & \texttt{eng} \texttt{spa} & \texttt{SO} & \texttt{ara}$^{\dagger}$ \texttt{som} \\
\texttt{AG} & \texttt{eng} & \texttt{DE} & \texttt{bar} \texttt{deu} \texttt{eng} \texttt{fra} \texttt{frr} \texttt{nds} & \texttt{IS} & \texttt{isl} & \texttt{MY} & \texttt{eng} \texttt{msa}$^{\dagger}$ \texttt{zho}$^{\dagger}$ & \texttt{SR} & \texttt{nld} \texttt{srn} \\
\texttt{AI} & \texttt{eng} & \texttt{DJ} & \texttt{aar} \texttt{ara}$^{\dagger}$ \texttt{fra} \texttt{som} & \texttt{IT} & \texttt{eng} \texttt{fra} \texttt{ita} \texttt{vec} & \texttt{MZ} & \texttt{por} \texttt{vmw} & \texttt{SS} & \texttt{ara}$^{\dagger}$ \texttt{eng} \\
\texttt{AL} & \texttt{sqi}$^{\dagger}$ & \texttt{DK} & \texttt{dan} \texttt{deu} \texttt{eng} \texttt{kal} \texttt{swe} & \texttt{JE} & \texttt{eng} & \texttt{NA} & \texttt{afr} \texttt{eng} \texttt{kua} \texttt{naq} \texttt{ndo} & \texttt{ST} & \texttt{fra} \texttt{por} \\
\texttt{AM} & \texttt{hye} & \texttt{DM} & \texttt{eng} & \texttt{JM} & \texttt{eng} \texttt{jam} & \texttt{NC} & \texttt{fra} & \texttt{SV} & \texttt{spa} \\
\texttt{AO} & \texttt{kmb} \texttt{por} \texttt{umb} & \texttt{DO} & \texttt{spa} & \texttt{JO} & \texttt{ara}$^{\dagger}$ \texttt{eng} & \texttt{NE} & \texttt{dje} \texttt{fra} \texttt{hau} & \texttt{SX} & \texttt{eng} \texttt{nld} \texttt{spa} \\
\texttt{AR} & \texttt{spa} & \texttt{DZ} & \texttt{ara}$^{\dagger}$ \texttt{arq} \texttt{fra} & \texttt{JP} & \texttt{jpn} & \texttt{NF} & \texttt{eng} & \texttt{SY} & \texttt{ara}$^{\dagger}$ \\
\texttt{AS} & \texttt{eng} \texttt{smo} & \texttt{EC} & \texttt{que}$^{\dagger}$ \texttt{spa} & \texttt{KE} & \texttt{eng} \texttt{kik} \texttt{luy}$^{\dagger}$ \texttt{swa}$^{\dagger}$ & \texttt{NG} & \texttt{eng} \texttt{hau} \texttt{ibo} \texttt{pcm} \texttt{yor} & \texttt{SZ} & \texttt{eng} \texttt{ssw} \\
\texttt{AT} & \texttt{bar} \texttt{deu} \texttt{eng} \texttt{fra} \texttt{hrv} \texttt{hun} \texttt{slv} & \texttt{EE} & \texttt{eng} \texttt{est}$^{\dagger}$ \texttt{fin} \texttt{rus} & \texttt{KG} & \texttt{kir} \texttt{rus} & \texttt{NI} & \texttt{spa} & \texttt{TC} & \texttt{eng} \\
\texttt{AU} & \texttt{eng} & \texttt{EG} & \texttt{ara}$^{\dagger}$ \texttt{eng} & \texttt{KH} & \texttt{khm} & \texttt{NL} & \texttt{deu} \texttt{eng} \texttt{fra} \texttt{fry} \texttt{nds} \texttt{nld} & \texttt{TD} & \texttt{ara}$^{\dagger}$ \texttt{fra} \\
\texttt{AW} & \texttt{nld} \texttt{pap} & \texttt{EH} & \texttt{ara}$^{\dagger}$ & \texttt{KI} & \texttt{eng} \texttt{gil} & \texttt{NO} & \texttt{nor}$^{\dagger}$ \texttt{sme} & \texttt{TG} & \texttt{ewe} \texttt{fra} \\
\texttt{AX} & \texttt{swe} & \texttt{ER} & \texttt{ara}$^{\dagger}$ \texttt{eng} \texttt{tig} \texttt{tir} & \texttt{KM} & \texttt{ara}$^{\dagger}$ \texttt{fra} \texttt{wni} \texttt{zdj} & \texttt{NP} & \texttt{mai} \texttt{nep}$^{\dagger}$ & \texttt{TH} & \texttt{eng} \texttt{tha} \texttt{tts} \\
\texttt{AZ} & \texttt{aze}$^{\dagger}$ & \texttt{ES} & \texttt{ast} \texttt{cat} \texttt{eng} \texttt{eus} \texttt{glg} \texttt{oci} \texttt{spa} & \texttt{KN} & \texttt{eng} & \texttt{NR} & \texttt{eng} \texttt{nau} & \texttt{TJ} & \texttt{rus} \texttt{tgk} \\
\texttt{BA} & \texttt{bos} \texttt{eng} \texttt{hrv} \texttt{srp} & \texttt{ET} & \texttt{amh} \texttt{eng} \texttt{orm}$^{\dagger}$ & \texttt{KP} & \texttt{kor} & \texttt{NU} & \texttt{eng} \texttt{niu} & \texttt{TK} & \texttt{eng} \texttt{smo} \texttt{tkl} \\
\texttt{BB} & \texttt{eng} & \texttt{FI} & \texttt{deu} \texttt{eng} \texttt{fin} \texttt{sms} \texttt{swe} & \texttt{KR} & \texttt{kor} & \texttt{NZ} & \texttt{eng} \texttt{mri} & \texttt{TL} & \texttt{por} \texttt{tet} \\
\texttt{BD} & \texttt{ben} \texttt{eng} & \texttt{FJ} & \texttt{eng} \texttt{fij} \texttt{hif} \texttt{hin} & \texttt{KW} & \texttt{ara}$^{\dagger}$ & \texttt{OM} & \texttt{ara}$^{\dagger}$ & \texttt{TM} & \texttt{rus} \texttt{tuk} \\
\texttt{BE} & \texttt{deu} \texttt{eng} \texttt{fra} \texttt{nld} \texttt{vls} & \texttt{FK} & \texttt{eng} & \texttt{KY} & \texttt{eng} & \texttt{PA} & \texttt{eng} \texttt{spa} & \texttt{TN} & \texttt{ara}$^{\dagger}$ \texttt{fra} \\
\texttt{BF} & \texttt{dyu} \texttt{fra} \texttt{mos} & \texttt{FM} & \texttt{chk} \texttt{eng} \texttt{pon} & \texttt{KZ} & \texttt{eng} \texttt{kaz} \texttt{rus} & \texttt{PE} & \texttt{que}$^{\dagger}$ \texttt{spa} & \texttt{TO} & \texttt{eng} \texttt{ton} \\
\texttt{BG} & \texttt{bul} \texttt{eng} \texttt{rus} \texttt{tur} & \texttt{FO} & \texttt{fao} & \texttt{LA} & \texttt{lao} & \texttt{PF} & \texttt{fra} \texttt{tah} & \texttt{TR} & \texttt{eng} \texttt{tur} \\
\texttt{BH} & \texttt{ara}$^{\dagger}$ & \texttt{FR} & \texttt{eng} \texttt{fra} \texttt{spa} & \texttt{LB} & \texttt{ara}$^{\dagger}$ \texttt{eng} \texttt{fra} & \texttt{PG} & \texttt{eng} \texttt{hmo} \texttt{tpi} & \texttt{TT} & \texttt{eng} \\
\texttt{BI} & \texttt{eng} \texttt{fra} \texttt{run} & \texttt{GA} & \texttt{fra} & \texttt{LC} & \texttt{eng} & \texttt{PH} & \texttt{ceb} \texttt{eng} \texttt{fil} \texttt{hil} \texttt{ilo} \texttt{mdh} \texttt{pag} \texttt{spa} \texttt{tsg} \texttt{war} & \texttt{TV} & \texttt{eng} \texttt{tvl} \\
\texttt{BJ} & \texttt{fon} \texttt{fra} & \texttt{GB} & \texttt{cym} \texttt{eng} \texttt{fra} \texttt{gla} \texttt{gle} & \texttt{LI} & \texttt{deu} \texttt{gsw} & \texttt{PK} & \texttt{eng} \texttt{lah} \texttt{pan} \texttt{pus}$^{\dagger}$ \texttt{skr} \texttt{snd} \texttt{urd} & \texttt{TW} & \texttt{zho}$^{\dagger}$ \\
\texttt{BL} & \texttt{fra} & \texttt{GD} & \texttt{eng} & \texttt{LK} & \texttt{eng} \texttt{sin} \texttt{tam} & \texttt{PL} & \texttt{csb} \texttt{deu} \texttt{eng} \texttt{lit} \texttt{pol} \texttt{rus} & \texttt{TZ} & \texttt{eng} \texttt{swa}$^{\dagger}$ \\
\texttt{BM} & \texttt{eng} & \texttt{GE} & \texttt{abk} \texttt{kat} \texttt{oss} \texttt{xmf} & \texttt{LR} & \texttt{eng} \texttt{kpe}$^{\dagger}$ & \texttt{PM} & \texttt{fra} & \texttt{UA} & \texttt{rus} \texttt{ukr} \\
\texttt{BN} & \texttt{msa}$^{\dagger}$ \texttt{zho}$^{\dagger}$ & \texttt{GF} & \texttt{fra} \texttt{gcr} & \texttt{LS} & \texttt{eng} \texttt{sot} \texttt{zul} & \texttt{PN} & \texttt{eng} & \texttt{UG} & \texttt{eng} \texttt{lug} \texttt{swa}$^{\dagger}$ \\
\texttt{BO} & \texttt{aym}$^{\dagger}$ \texttt{que}$^{\dagger}$ \texttt{spa} & \texttt{GG} & \texttt{eng} & \texttt{LT} & \texttt{deu} \texttt{eng} \texttt{lit} \texttt{rus} & \texttt{PR} & \texttt{eng} \texttt{spa} & \texttt{US} & \texttt{eng} \texttt{haw} \texttt{spa} \\
\texttt{BQ} & \texttt{nld} \texttt{pap} & \texttt{GH} & \texttt{aka} \texttt{eng} \texttt{ewe} \texttt{gaa} & \texttt{LU} & \texttt{deu} \texttt{eng} \texttt{fra} \texttt{ltz} \texttt{por} & \texttt{PS} & \texttt{ara}$^{\dagger}$ & \texttt{UY} & \texttt{spa} \\
\texttt{BR} & \texttt{por} \texttt{vec} & \texttt{GI} & \texttt{eng} \texttt{spa} & \texttt{LV} & \texttt{eng} \texttt{lav}$^{\dagger}$ \texttt{rus} & \texttt{PT} & \texttt{eng} \texttt{fra} \texttt{por} \texttt{spa} & \texttt{UZ} & \texttt{rus} \texttt{uzb}$^{\dagger}$ \\
\texttt{BS} & \texttt{eng} & \texttt{GL} & \texttt{dan} \texttt{kal} & \texttt{LY} & \texttt{ara}$^{\dagger}$ & \texttt{PW} & \texttt{eng} \texttt{pau} & \texttt{VA} & \texttt{ita} \texttt{lat} \\
\texttt{BT} & \texttt{dzo} \texttt{eng} \texttt{nep}$^{\dagger}$ \texttt{tsj} & \texttt{GM} & \texttt{eng} \texttt{man}$^{\dagger}$ & \texttt{MA} & \texttt{ara}$^{\dagger}$ \texttt{eng} \texttt{fra} \texttt{tzm} \texttt{zgh} & \texttt{PY} & \texttt{grn}$^{\dagger}$ \texttt{spa} & \texttt{VC} & \texttt{eng} \\
\texttt{BW} & \texttt{eng} \texttt{tsn} & \texttt{GN} & \texttt{fra} \texttt{ful}$^{\dagger}$ \texttt{man}$^{\dagger}$ \texttt{sus} & \texttt{MC} & \texttt{fra} & \texttt{QA} & \texttt{ara}$^{\dagger}$ \texttt{fas}$^{\dagger}$ & \texttt{VE} & \texttt{spa} \\
\texttt{BY} & \texttt{bel} \texttt{rus} & \texttt{GP} & \texttt{fra} & \texttt{MD} & \texttt{ron} \texttt{ukr} & \texttt{RE} & \texttt{fra} \texttt{rcf} \texttt{tam} & \texttt{VG} & \texttt{eng} \\
\texttt{BZ} & \texttt{eng} \texttt{spa} & \texttt{GQ} & \texttt{fan} \texttt{fra} \texttt{por} \texttt{spa} & \texttt{ME} & \texttt{srp} & \texttt{RO} & \texttt{eng} \texttt{fra} \texttt{ron} \texttt{spa} & \texttt{VI} & \texttt{eng} \\
\texttt{CA} & \texttt{chp} \texttt{crk} \texttt{den} \texttt{dgr} \texttt{eng} \texttt{fra} \texttt{gwi} \texttt{iku} & \texttt{GR} & \texttt{ell} \texttt{eng} & \texttt{MF} & \texttt{fra} & \texttt{RS} & \texttt{hrv} \texttt{hun} \texttt{ron} \texttt{slk} \texttt{sqi}$^{\dagger}$ \texttt{srp} \texttt{ukr} & \texttt{VN} & \texttt{vie} \\
\texttt{CD} & \texttt{fra} \texttt{kon} \texttt{lin} \texttt{lua} \texttt{swa}$^{\dagger}$ & \texttt{GT} & \texttt{quc} \texttt{spa} & \texttt{MG} & \texttt{eng} \texttt{fra} \texttt{mlg}$^{\dagger}$ & \texttt{RU} & \texttt{ady} \texttt{ava} \texttt{aze}$^{\dagger}$ \texttt{bak} \texttt{che} \texttt{inh} \texttt{kbd} \texttt{koi} \texttt{kom} \texttt{krc} \texttt{kum} \texttt{lbe} \texttt{lez} \texttt{mdf} \texttt{myv} \texttt{rus} \texttt{sah} \texttt{tat} \texttt{tyv} \texttt{udm} & \texttt{VU} & \texttt{bis} \texttt{eng} \texttt{fra} \\
\texttt{CF} & \texttt{fra} \texttt{sag} & \texttt{GU} & \texttt{cha} \texttt{eng} & \texttt{MH} & \texttt{eng} \texttt{mah} & \texttt{RW} & \texttt{eng} \texttt{fra} \texttt{kin} & \texttt{WF} & \texttt{fra} \texttt{fud} \texttt{wls} \\
\texttt{CG} & \texttt{fra} & \texttt{GW} & \texttt{fra} \texttt{por} & \texttt{MK} & \texttt{mkd} \texttt{sqi}$^{\dagger}$ & \texttt{SA} & \texttt{ara}$^{\dagger}$ & \texttt{WS} & \texttt{eng} \texttt{smo} \\
\texttt{CH} & \texttt{deu} \texttt{eng} \texttt{fra} \texttt{gsw} \texttt{ita} \texttt{roh} & \texttt{GY} & \texttt{eng} & \texttt{ML} & \texttt{bam} \texttt{fra} & \texttt{SB} & \texttt{eng} \texttt{pis} & \texttt{XK} & \texttt{sqi}$^{\dagger}$ \texttt{srp} \\
\texttt{CI} & \texttt{bci} \texttt{fra} & \texttt{HK} & \texttt{eng} \texttt{zho}$^{\dagger}$ & \texttt{MM} & \texttt{mya} & \texttt{SC} & \texttt{crs} \texttt{eng} \texttt{fra} & \texttt{YE} & \texttt{ara}$^{\dagger}$ \\
\texttt{CK} & \texttt{eng} & \texttt{HN} & \texttt{spa} & \texttt{MN} & \texttt{mon}$^{\dagger}$ & \texttt{SD} & \texttt{apd} \texttt{ara}$^{\dagger}$ \texttt{eng} & \texttt{YT} & \texttt{buc} \texttt{fra} \texttt{swb} \\
\texttt{CL} & \texttt{spa} & \texttt{HR} & \texttt{eng} \texttt{hrv} \texttt{ita} \texttt{vec} & \texttt{MO} & \texttt{eng} \texttt{por} \texttt{zho}$^{\dagger}$ & \texttt{SE} & \texttt{eng} \texttt{fin} \texttt{swe} & \texttt{ZA} & \texttt{afr} \texttt{eng} \texttt{nbl} \texttt{nso} \texttt{sot} \texttt{ssw} \texttt{tsn} \texttt{tso} \texttt{ven} \texttt{xho} \texttt{zul} \\
\texttt{CM} & \texttt{eng} \texttt{fra} & \texttt{HT} & \texttt{fra} \texttt{hat} & \texttt{MP} & \texttt{cha} \texttt{eng} & \texttt{SG} & \texttt{eng} \texttt{msa}$^{\dagger}$ \texttt{tam} \texttt{zho}$^{\dagger}$ & \texttt{ZM} & \texttt{bem} \texttt{eng} \texttt{nya} \texttt{toi} \\
\texttt{CN} & \texttt{bod} \texttt{kor} \texttt{mon}$^{\dagger}$ \texttt{uig} \texttt{zha} \texttt{zho}$^{\dagger}$ & \texttt{HU} & \texttt{deu} \texttt{eng} \texttt{hun} & \texttt{MQ} & \texttt{fra} & \texttt{SH} & \texttt{eng} & \texttt{ZW} & \texttt{eng} \texttt{nde} \texttt{sna} \\
\texttt{CO} & \texttt{spa} & \texttt{ID} & \texttt{ind} \texttt{jav} \texttt{sun} & \texttt{MR} & \texttt{ara}$^{\dagger}$ \texttt{fra} & \texttt{SI} & \texttt{deu} \texttt{eng} \texttt{hrv} \texttt{slv} \texttt{vec} &  &  \\
\texttt{CR} & \texttt{spa} & \texttt{IE} & \texttt{eng} \texttt{fra} \texttt{gle} & \texttt{MS} & \texttt{eng} & \texttt{SJ} & \texttt{nob} \texttt{rus} &  &  \\
\texttt{CU} & \texttt{spa} & \texttt{IL} & \texttt{ara}$^{\dagger}$ \texttt{eng} \texttt{heb} \texttt{rus} & \texttt{MT} & \texttt{eng} \texttt{fra} \texttt{ita} \texttt{mlt} & \texttt{SK} & \texttt{ces} \texttt{deu} \texttt{eng} \texttt{hun} \texttt{slk} &  &  \\
\texttt{CV} & \texttt{kea} \texttt{por} & \texttt{IM} & \texttt{eng} \texttt{glv} & \texttt{MU} & \texttt{eng} \texttt{fra} \texttt{mfe} & \texttt{SL} & \texttt{eng} \texttt{kri} \texttt{men} \texttt{tem} &  &  \\
\bottomrule
\end{tabular}
\caption{Main languages per country used for the main-language analyses
(Appendix~\ref{app:robustness-mainlang}). A language counts as a main
language of a country if, in CLDR territory--language data, it has official
status (official, de facto official, or official regional) or a speaker share
of at least 10\%; ISO 639-3 codes, countries as ISO 3166-1 alpha-2.
Macrolanguage codes marked $^{\dagger}$ additionally stand for their
individual-variety codes in the corpus locale naming (e.g.\ \texttt{ara}
covers \texttt{arb}, \texttt{arz}, \texttt{ary}, \ldots).}
\label{tab:country-languages}
\end{table*}

